VISAR: A Human-AI Argumentative Writing Assistant with Visual Programming and Rapid Draft Prototyping

In argumentative writing, writers must brainstorm hierarchical writing goals, ensure the persuasiveness of their arguments, and revise and organize their plans through drafting. Recent advances in large language models (LLMs) have made interactive text generation through a chat interface (e.g., ChatGPT) possible. However, this approach often neglects implicit writing context and user intent, lacks support for user control and autonomy, and provides limited assistance for sensemaking and revising writing plans. To address these challenges, we introduce VISAR, an AI-enabled writing assistant system designed to help writers brainstorm and revise hierarchical goals within their writing context, organize argument structures through synchronized text editing and visual programming, and enhance persuasiveness with argumentation spark recommendations. VISAR allows users to explore, experiment with, and validate their writing plans using automatic draft prototyping. A controlled lab study confirmed the usability and effectiveness of VISAR in facilitating the argumentative writing planning process.

==> paper/3_design_goals.tex <==
\section{Design Goals}

Given the various stages involved in \argu, we set our system's design goal as follows:

- support higher-level planning and outlining with less need to worry about writing intricacies (e.g. detailed arguments and stuff) --> agent
- quickly prototype and validate ideas in \argu --> agent
- clearly visualize paragraph structures
- support lower-level direct drafting as part of the natural writing process    --> direct manipulation

% From the cognitive perspective, writing process can be decomposed into several stages, including planning, drafting, rewriting or revising, editing, and reviewing \cite{flower1981cognitive, yang2022re3}.
% During the planning stage, the writer retrieves relevant information from their long-term memory and generates ideas based on their prior knowledge of the topic. This involves creating an outline, setting, and characters to organize the writing.

